Informative Image Captioning with External Sources of Information

An image caption should fluently present the essential information in a given image, including informative, fine-grained entity mentions and the manner in which these entities interact. However, current captioning models are usually trained to generate captions that only contain common object names, thus falling short on an important "informativeness" dimension. We present a mechanism for integrating image information together with fine-grained labels (assumed to be generated by some upstream models) into a caption that describes the image in a fluent and informative manner. We introduce a multimodal, multi-encoder model based on Transformer that ingests both image features and multiple sources of entity labels. We demonstrate that we can learn to control the appearance of these entity labels in the output, resulting in captions that are both fluent and informative.

==> results-table-3sys.tex <==
\begin{table*}[h]
    \fontsize{8}{10}\selectfont
    \begin{tabular}{c|cc|ccc|ccc|ccc}
    \hline
    \multicolumn{3}{c|}{Input Configuration} &
      \multicolumn{3}{c|}{DeepRanking CNN model} &
      \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}ResNet CNN model \\ trained on ImageNet\end{tabular}} &
      \multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}ResNet CNN model \\ trained on JFT\end{tabular}} \\ \hline
    \begin{tabular}{p{0.08\textwidth}}Web Entity\end{tabular} &
      $W^{recall}_{we}$ &
      $W^{prec}_{obj}$  &
      CIDEr             &
      $S^{recall}_{we}$ &
      $S^{prec}_{obj}$  &
      CIDEr             &
      $S^{recall}_{we}$ &
      $S^{prec}_{obj}$  &
      CIDEr             &
      $S^{recall}_{we}$ &
      $S^{prec}_{obj}$ \\ \hline
    Type  & \colorbox{yellow}{1.0}  & \colorbox{green}{1.0}  & 68.06 & \colorbox{yellow}{38.78} & \colorbox{green}{7.82} & 69.46  & \colorbox{yellow}{36.80}  & \colorbox{green}{6.93} & 74.60 & \colorbox{yellow}{40.39} & \colorbox{green}{6.87} \\
    Type  & \colorbox{yellow}{1.5}  & 1.0  &  63.93 & \colorbox{yellow}{41.91} & 8.00 & 65.41  & \colorbox{yellow}{39.65}  & 7.00 & 70.81 & \colorbox{yellow}{42.95} & 7.04  \\
    Type  & 1.0  & \colorbox{green}{1.5}  &  65.54 & 38.81 & \colorbox{green}{9.73} & 68.01  & 36.45  & \colorbox{green}{8.87} & 73.82 & 40.03 & \colorbox{green}{8.38} \\
    Type  & 1.5  & 1.5  &  60.58 & 41.68 & 9.73 & 65.30  & 38.97  & 8.81 & 71.11 & 41.94 & 8.48 \\
    \hline
    Name  & \colorbox{yellow}{1.0}  & \colorbox{green}{1.0}  &  \bf{80.21} & \colorbox{yellow}{31.08} & \colorbox{green}{6.62} & \bf{80.69}  & \colorbox{yellow}{31.15}  & \colorbox{green}{6.19} & \bf{87.25} & \colorbox{yellow}{31.01} & \colorbox{green}{6.27} \\
    Name  & \colorbox{yellow}{1.5}  & 1.0  &  76.78 & \colorbox{yellow}{37.32} & 6.96 & 76.53  & \colorbox{yellow}{38.20}  & 6.13 & 83.62 & \colorbox{yellow}{38.08} & 6.76 \\
    Name  & 1.0  & \colorbox{green}{1.5}  &  76.97 & 31.18 & \colorbox{green}{8.00} & 76.05  & 30.72  & \colorbox{green}{6.91} & 83.34 & 30.64 & \colorbox{green}{7.74} \\
    Name  & 1.5  & 1.5  &  75.94 & 37.41 & 8.24 & 75.76  & 38.02  & 7.23 & 82.18 & 38.17 & 7.93 \\ \hline
    \end{tabular}
    \caption {
        Variants of our proposed approach using \emph{both} image and entity labels.
        We present ablations on the CNN model \& pretraining conditions, on the coverage boost factors $W^{recall}_{we}$ and $W^{prec}_{obj}$, and entity label modeling (type-only versus surface-form names).
        We measure CIDEr and output label coverage metrics (higher value indicates better performance).
        We see that all models learn to increase the coverage of input labels in the output caption as the coverage boost factors are increased (correlations highlighed in yellow and green, resp.).
        Note that type-only models generally have a higher label coverage compared to using surface-forms directly.
        CIDEr does not correlate with coverage gains, because the input labels often do not appear in the ground-truth captions (first row).
        However, human evaluation does correlate accuracy with coverage gains (Table~\ref{tab:human_eval})).}
    \label{tab:quant}
\end{table*}

